A Data-driven Hierarchical Control Structure for Systems with Uncertainty

The paper introduces a Data-driven Hierarchical Control (DHC) structure to improve performance of systems operating under the effect of system and/or environment uncertainty. The proposed hierarchical approach consists of two parts: 1) A data-driven model identification component to learn a linear approximation between reference signals given to an existing lower-level controller and uncertain time-varying plant outputs. 2) A higher-level controller component that utilizes the identified approximation and wraps around the existing controller for the system to handle modeling errors and environment uncertainties during system deployment. We derive loose and tight bounds for the identified approximation's sensitivity to noisy data. Further, we show that adding the higher-level controller maintains the original system's stability. A benefit of the proposed approach is that it requires only a small amount of observations on states and inputs, and it thus works online; that feature makes our approach appealing to robotics applications where real-time operation is critical. The efficacy of the DHC structure is demonstrated in simulation and is validated experimentally using aerial robots with approximately-known mass and moment of inertia parameters and that operate under the influence of ground effect.

==> modeling.tex <==
\section{Modeling Experiments}
We show the efficiency of the method introduced in section II-A by identifying models online and giving associated predictions. We begin with a toy example that considers a linear system, and then move on to process data from a Hummingbird quadrotor flying under the influence of ground effect. 

\subsection{Toy Example: Linear System}
The theory is implemented in the linear system (8). The data matrices constructed from computing the first three temporal snapshots when a random input sequence is given are
$$X = \left[
          \begin{matrix}
            1&4&21 \\
            1&8&44 \\
          \end{matrix} 
          \right], \enspace X_p = \left[
          \begin{matrix}
            4&21&112 \\
            8&44&242 \\
          \end{matrix} 
          \right],$$
          $$U = \left[
          \begin{matrix}
            1&2&2\\
          \end{matrix} 
          \right].$$

         
          
Using the $linsolve$ command in MATLAB R2018b, the estimated model is 
$$\hat{A}=\left[
          \begin{matrix}
            1&2 \\
           3&4  \\
          \end{matrix} 
          \right]\enspace\text{,}\enspace \hat{B} =\left[
          \begin{matrix}
            1 \\
           0.7  \\
          \end{matrix} 
          \right] $$
          
As shown above, for a linear system, we can reconstruct the system exactly with data of only $K_e=n+m+1$ steps. 
%\subsection{Nonlinear system}
%For nonlinear systems, MIM identify and update the model of original dynamics through linearizing at every $K_e+1$ steps. Several methods have been developed to transform a nonlinear system into an equivalent linear system, here we will compare our method with the linearized model obtained by linearizing at the equilibrium points (LEP). 

%\begin{figure}
%\centering
%\includegraphics[width = 0.3\textwidth]{pendulum.png}
%\caption{\label{RefinedMiC} Two-dimensional inverted pendulum}
%\end{figure}
%We implemented them in an nonlinear inverted pendulum model as depicted in Fig \ref{RefinedMiC}. Its model can be described as:
%$$\begin{cases}
%    (M+m) \ddot{x}+b \dot{x}+m l \ddot{\theta} \cos \theta-m l \dot{\theta}^{2} \sin \theta=F\\
%    \left(I+m l^{2}\right) \ddot{\theta}+m g l \sin \theta=-m l \ddot{x} \cos \theta
%\end{cases}$$

%In that experiment, $m = 0.2kg$, $M = 0.5kg$, $l = 0.3m$, $I = 0.006kg m^2$, $b = 0.1M/m/s$, $g = 9.8M/s^2$. We 
% \begin{figure*}
%\centering
%\includegraphics[width = 0.5\textwidth]{nonpre.png}\includegraphics[width = 0.5\textwidth]{nonpre_no.png}
%\caption{\label{fig:10} True states (blue) and predictions of nonlinear inverted pendulum generated by MIM (red) and LEP (yellow) (left: a1, right: a2).}
%\end{figure*} 
%evolved the system for 40 steps with a simple PID controller and gathered observed states and inputs. These data are used to identify model and give prediction. In the first case (a1), we propagate the system without external influence and add a random uncertainty to states in the second case (a2). The results of prediction are shown in Fig \ref{fig:10}.

%Results suggest that LEP can produce an accurate prediction of states except $\dot{\theta}$ when no uncertainty are added, but it would generate more error when disturbances are combined. While MIM can model the nonlinear system and give corresponding predictions accurately in both cases.
\subsection{Modeling a Hummingbird Quadrotor}

We use an AscTec Hummingbird quadrotor tasked to hover at four specific distances from the ground  $h = \{ 2,\ 11,\ 20,\ 50\}$\;cm under ground effect and collect the corresponding experimental data. %The data are used to train models that relate heights to sequences. Then we do prediction for a new height within 2cm to 50cm through linear combination of corresponding sequences. Details is introduced in \cite{c6}.
%
Nylon cord is attached to the support structure to constrain the problem in one dimension as illustrated in Fig.~\ref{hum}. The data set contains 250 trials for each case, logged at $30$\;fps for a total of $15$\;sec. After normalization, there are $441$ snapshots in each time sequence. Data are used to train a model based on our proposed approach, and to train a model~\cite{c6} based on Proper Orthogonal Decomposition~\cite{c5}, as well as several shallow neural networks for comparison. We note here that POD is used for data analysis aimed at obtaining low-dimensional approximate descriptions of a high-dimensional process. It can decompose the system into principal dynamic modes consisting of principal spatial and temporal modes that store the largest possible amount of energy. Unfortunately, derived models are implicit and thus difficult to be implemented for control. (Details can be found in \cite{c5} and \cite{c6}.) As for shallow neural networks, we train two types of recurrent neural networks (RNNs): gated recurrent units (GRUs) and long short-term memory (LSTMs) with different parameters. 

\begin{figure}
\vspace{6pt}
\centering
\includegraphics[width = 0.24\textwidth, trim=10 0 10 60, clip]{Humming.png}
\vspace{-3pt}
\caption{The Hummingbird quadrotor commanded to hover at a certain height.}
\label{hum}
\vspace{-6pt}
\end{figure}

Table \ref{tab2} represents the comparison on efficiency among these methods. The running time here refers to the total time for training and prediction. The average loss is defined using the mean squared error $L=\frac{1}{N} \sum _{k=1}^N(v(k)-\hat{v}(k))^2$. As the table indicates, our method has the highest accuracy among the other methods while working with limited data. As for running time, although POD attains the shortest time, our method's running time is significantly smaller than the running times of RNN networks. These results show our method's efficacy both in terms of accuracy and efficiency.
%
\begin{table}[h]
\caption{Prediction comparison in Hummingbird quadrotor}
\label{tab2}
\begin{center}
\scalebox{.9}{
\begin{tabular}{|c|c|c|c|}
\hline
Type of Methods & Optimal LR& Average Loss & Running Time(s)\\
\hline
POD & $\backslash$ & 0.1926 & 1.8316 \\
\hline
Our method* & $\backslash$ & 0.0866 & 2.2113  \\
\hline
SGD[32,relu] & $0.0001$ & 23.2563 & 133.3804 \\
\hline
RMSprop[32,relu] & $0.001$ & 110.7220 & 134.4922  \\
\hline
Adam[32,relu] & $\backslash$ & 31.4722 & 669.0302  \\
\hline
SGD[64,relu] & $0.001$ & 6.0806 & 632.2900  \\
\hline
RMSprop[32,relu] & $0.0001$ & 211.5433 & 646.4543  \\
\hline
SGD[32,relu6] & $0.001$ & 10.6723 & 269.5306  \\
\hline
RMSprop[32,relu6] & $0.001$ & 8.6456 & 234.7573  \\
\hline
\end{tabular}
}
\end{center}
\end{table}
